Consolidating Ranking and Relevance Predictions of Large Language Models through Post-Processing

The powerful generative abilities of large language models (LLMs) show potential in generating relevance labels for search applications. Previous work has found that directly asking about relevancy, such as ``How relevant is document A to query Q?", results in sub-optimal ranking. Instead, the pairwise ranking prompting (PRP) approach produces promising ranking performance through asking about pairwise comparisons, e.g., ``Is document A more relevant than document B to query Q?". Thus, while LLMs are effective at their ranking ability, this is not reflected in their relevance label generation. In this work, we propose a post-processing method to consolidate the relevance labels generated by an LLM with its powerful ranking abilities. Our method takes both LLM generated relevance labels and pairwise preferences. The labels are then altered to satisfy the pairwise preferences of the LLM, while staying as close to the original values as possible. Our experimental results indicate that our approach effectively balances label accuracy and ranking performance. Thereby, our work shows it is possible to combine both the ranking and labeling abilities of LLMs through post-processing.

==> background.tex <==
\section{Background: Piecewise linear transformation}\label{sec:background}
A common technique to post-process the unbounded ranking scores is the 
piecewise linear transformation (PWL)~\cite{ravina2021distilling} or Platt-scaling for binary labels~\cite{PlattScaling:1999}. 
In this method, given ranking scores $s$, we leverage some labelled data to fit for a monotonic transform function $f(s)$, so that the mean squared error in \eqnref{eq:mse} between $f(s)$ and the golden label $y$ is minimized. 

In specific, the PWL defines the transformation function $f$ as:
\begin{align}
\label{eq:pwl}
    &f\big(s \mid \{\tilde{s}_m, \tilde{y}_m\}_{m=1}^M\big) = \\
    &\quad\begin{cases}
        \tilde{y}_1 & s\leq \tilde{s}_1, \\
        \tilde{y}_m + \frac{\tilde{y}_{m+1} - \tilde{y}_m}{\tilde{s}_{m+1} - \tilde{s}_m}(s - \tilde{s}_m)
        & \tilde{s}_m < s\leq \tilde{s}_{m+1}, \\
        \tilde{y}_M & s> \tilde{s}_M, 
    \end{cases}
    \nonumber
\end{align}
where $\{\tilde{s}_m, \tilde{y}_m\}_{m=1}^M$ are $2M$ fitting parameters.

In the case of binary labels, a binary cross entropy loss is typically applied to the Platt-scaling:
%
\begin{equation}
\label{eq:platt}
    f(s \mid {\alpha, \beta}) = \frac{1}{1+\exp[-(\alpha s +\beta)]},
\end{equation}
%
with $\alpha$ and $\beta$ fitting parameters.
To reinforce the monotonicity of the transformation, $\tilde{y}_{m+1} > \tilde{y}_m$ and $\tilde{s}_{m+1} > \tilde{s}_m$ are enforced for any $m$ in PWL and $\alpha > 0$ in Platt scaling.
Consequently, neither transformation can change the ranking of candidates, thereby, they allow us to improve relevance prediction performance without ever affecting the ranking performance.

However, PWL-like methods alone may not be sufficient to fully consolidate the ranking and relevance predictions of LLMs for two main reasons:
Firstly, it requires ground truth labels to be available on a reasonable amount of representative data, which is unlikely when there is a need for using LLMs as labellers.
Secondly, PWL-like transformations only consider the PRP predictions $s$ and never the pointwise relevance predictions $\hat{y}$, neither during training nor inference.
Therefore, they are not actually consolidating these two types of prediction, but merely aiming to increase the relevance prediction performance of PRP based on ground truth labels.

%the performance of using post-processed scores as relevance labels is bounded by not compromising any ranking performance as the relative order is preserved in such transformations.

